Application-Based Coexistence of Different Waveforms on Non-orthogonal Multiple Access

The coexistence of different wireless communication systems such as LTE and Wi-Fi by sharing the unlicensed band is well studied in the literature. In these studies, various methods are proposed to support the coexistence of systems, including listen-before-talk mechanism, joint user association and resource allocation. However, in this study, the coexistence of different waveform structures in the same resource elements are studied under the theory of non-orthogonal multiple access. This study introduces a paradigm-shift on NOMA towards the application-centric waveform coexistence. Throughout the paper, the coexistence of different waveforms is explained with two specific use cases, which are power-balanced NOMA and joint radar-sensing and communication with NOMA. In addition, some of the previous works in the literature regarding non-orthogonal waveform coexistence are reviewed. However, the concept is not limited to these use cases. With the rapid development of wireless technology, next-generation wireless systems are proposed to be flexible and hybrid, having different kinds of capabilities such as sensing, security, intelligence, control, and computing. Therefore, the concept of different waveforms' coexistence to meet these concerns are becoming impressive for researchers.

==> Waveform_Coexistence 2/acros.tex <==
% Extend acronym package with first letter caps
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother
% Acronyms
\acrodef{ofdm}[OFDM]{orthogonal frequency division multiplexing}
\acrodef{fofdm}[F-OFDM]{filtered-\aclu{ofdm}}
\acrodef{fbmc}[FBMC]{filter bank multicarrier}
\acrodef{fmt}[FMT]{filtered multitone}
\acrodef{ufmc}[UFMC]{universal filtered multicarrier}
\acrodef{gfdm}[GFDM]{generalized frequency division multiplexing}
\acrodef{zf}[ZF]{zero forcing}
\acrodef{mimo}[MIMO]{multiple-input multiple-output}
\acrodef{siso}[SISO]{single-input single-output}
\acrodef{np}[NP]{nondeterministic polynomial}
\acrodef{sc}[SC]{single carrier}
\acrodef{sc-fde}[SC-FDE]{\aclu{sc}-\aclu{fde}}
\acrodef{evm}[EVM]{error vector magnitude}
\acrodef{dft}[DFT]{discrete Fourier transformation}
\acrodef{ifft}[IFFT]{inverse fast Fourier transformation}
\acrodef{cp}[CP]{cyclic prefix}
\acrodef{papr}[PAPR]{peak-to-average power ratio}
\acrodef{qam}[QAM]{quadrature amplitude modulation}
\acrodef{ask}[ASK]{amplitude shift keying}
\acrodef{psk}[PSK]{phase shift keying}
\acrodef{apsk}[APSK]{amplitude phase shift keying}
\acrodef{fsk}[FSK]{frequency shift keying}
\acrodef{gmsk}[GMSK]{gaussian minimum shift keying}
\acrodef{im}[IM]{index modulation}
\acrodef{fft}[FFT]{fast Fourier transformation}
\acrodef{ici}[ICI]{inter-carrier interference}
\acrodef{isi}[ISI]{intersymbol interference}
\acrodef{ini}[INI]{inter-numerology interference}
\acrodef{pdf}[PDF]{probability density function}
\acrodef{cr}[CR]{cognitive radio}
\acrodef{wola}[WOLA]{weighted overlap-add}
\acrodef{qos}[QoS]{Quality of Service}
\acrodef{csi}[CSI]{channel state information}
\acrodef{ber}[BER]{bit-error rate}
\acrodef{rf}[RF]{radio frequency}
\acrodef{rrc}[RRC]{root-raised cosine}
\acrodef{as}[AS]{alignment signal}
\acrodef{snr}[SNR]{signal-to-noise ratio}
\acrodef{dfe}[DFE]{decision-feedback equalizer}
\acrodef{fde}[FDE]{frequency domain equalization}
\acrodef{oob}[OOB]{out-of-band}
\acrodef{aci}[ACI]{adjacent channel interference}
\acrodef{naci}[NACI]{noise-plus-\aclu{aci}}
\acrodef{phy}[PHY]{physical layer}
\acrodef{mse}[MSE]{mean-square error}
\acrodef{pa}[PA]{power amplifier}
\acrodef{rb}[RB]{resource block}
\acrodef{ran}[RAN]{radio-access network}
\acrodef{rat}[RAT]{radio access technology}
\acrodefplural{rat}[RATs]{radio access technologies}
\acrodef{mmwave}[mmWave]{millimeter wave}
\acrodef{3gpp}[3GPP]{Third Generation Partnership Project}
\acrodef{sc}[SC]{single carrier}
\acrodef{uw}[UW]{unique word}
\acrodef{zt}[ZT]{zero tail}
\acrodef{gi}[GI]{guard interval}
\acrodef{sinr}[SINR]{signal to interference plus noise ratio}
\acrodef{dpss}[DPSS]{discrete prolate spheroidal sequences}
\acrodef{bler}[BLER]{block error rate}
\acrodef{fdd}[FDD]{frequency domain duplexing}
\acrodef{tdd}[TDD]{time domain duplexing}
\acrodef{ul}[UL]{uplink}
\acrodef{dl}[DL]{downlink}
\acrodef{bs}[BS]{base station}
\acrodef{af}[AF]{ambiguity function}
\acrodef{ms}[MS]{mobile station}
\acrodef{iot}[IoT]{Internet of Things}
\acrodef{pdp}[PDP]{power delay profile}
\acrodef{ftn}[FTN]{Faster-than-Nyquist}
\acrodef{svd}[SVD]{singular-value decomposition}
\acrodef{uw-ofdm}[UW-OFDM]{\aclu{uw}-\aclu{ofdm}}
\acrodef{w-ofdm}[W-OFDM]{windowed-\aclu{ofdm}}
\acrodef{rw-ofdm}[RW-OFDM]{receiver \aclu{w-ofdm}}
\acrodef{cp-ofdm}[CP-OFDM]{\aclu{cp}-\aclu{ofdm}}
\acrodef{dft-s-ofdm}[DFT-s-OFDM]{\aclu{dft}-spread-\aclu{ofdm}}
\acrodef{lte}[LTE]{Long Term Evolution}
\acrodef{lte-a}[LTE-A]{\aclu{lte}-Advanced}
\acrodef{gsm}[GSM]{Global System for Mobile Communications}
\acrodef{ma}[MA]{multiple accessing}
\acrodef{oma}[OMA]{orthogonal multiple access}
\acrodef{noma}[NOMA]{non-orthogonal multiple access}
\acrodef{cdnoma}[CD-NOMA]{code domain \aclu{noma}}
\acrodef{pdnoma}[PD-NOMA]{power domain \aclu{noma}}
\acrodef{fdma}[FDMA]{frequency division multiple accessing}
\acrodef{ofdma}[OFDMA]{orthogonal frequency division multiple accessing}
\acrodef{sc-fdma}[SC-FDMA]{single carrier-frequency division multiple accessing}
\acrodef{cdma}[CDMA]{code division multiple access}
\acrodef{tdma}[TDMA]{time division multiple access}
\acrodef{embb}[eMBB]{enhanced-mobile broadband}
\acrodef{mmtc}[mMTC]{massive machine type communications}
\acrodef{urllc}[uRLLC]{ultra-reliable and low-latency communications}
\acrodef{dvb}[DVB]{digital video broadcasting}
\acrodef{comp}[CoMP]{Coordinated Multi Point}
\acrodef{jt-comp}[JT-CoMP]{Joint Transmission-\aclu{comp}}
\acrodef{sic}[SIC]{successive interference cancellation}
\acrodef{osic}[OSIC]{ordered successive interference cancellation}
\acrodef{ml}[ML]{maximum likelihood}
\acrodef{mud}[MUD]{multi-user detection}
\acrodef{mlmud}[ML-MUD]{maximum likelihood multi-user detection}
\acrodef{sl}[SL]{sidelink}
\acrodef{qpsk}[QPSK]{quadrature phase shift keying}
\acrodef{mpa}[MPA]{message passing algorithm}
\acrodef{amc}[AMC]{adaptive modulation and coding}
\acrodef{umts}[UMTS]{Universal Mobile Telecommunications Service}
\acrodef{e-utra}[E-UTRA]{Evolved \aclu{umts} Terrestrial Radio Access}
\acrodef{ue}[UE]{user equipment}
\acrodef{harq}[HARQ]{hybrid automatic repeat request}
\acrodef{nr}[NR]{new radio}
\acrodef{hetnet}[HetNet]{heterogeneous network}
\acrodef{pot}[POT]{partially overlapping tones}
\acrodef{rms}[RMS]{root mean square}
\acrodef{must}[MUST]{multiuser superposition transmission}
\acrodef{csma}[CSMA]{carrier sense \aclu{ma}}
\acrodef{sdma}[SDMA]{space division \aclu{ma}}
\acrodef{mno}[MNO]{mobile network operator}
\acrodef{d2d}[D2D]{device-to-device}
\acrodef{v2v}[V2V]{vehicle-to-vehicle}
\acrodef{v2x}[V2X]{vehicle-to-infrastructure}
\acrodef{med}[MED]{maximum excess delay}
\acrodef{awgn}[AWGN]{additive white Gaussian noise}
\acrodef{cfr}[CFR]{channel frequency response}
\acrodef{cir}[CIR]{channel impulse response}
\acrodef{sir}[SIR]{signal-to-interference ratio}
\acrodef{lut}[LUT]{lookup table}
\acrodef{ssw}[SSW]{subcarrier specific window}
\acrodef{cqi}[CQI]{channel quality indicator}
\acrodef{bpsk}[BPSK]{binary phase shift keying}
\acrodef{mcs}[MCS]{modulation and coding scheme}
\acrodef{dac}[DAC]{digital-to-analog converter}
\acrodef{ncofdm}[NC-OFDM]{$N$-Continuous \aclu{ofdm}}
\acrodef{adc}[ADC]{analog-to-digital converter}
\acrodef{e2e}[E2E]{end-to-end}
\acrodef{kpi}[KPI]{key performance indicator}
\acrodef{p1db}[P1dB]{1 dB compression point}
\acrodef{sqnr}[SQNR]{signal-to-quantization-noise ratio}
\acrodef{cmos}[CMOS]{complementary metal–oxide–semiconductor}
\acrodef{cs}[CS]{cyclic suffix}
\acrodef{pn}[PN]{phase noise}
\acrodef{xo}[XO]{crystal oscillator}
\acrodef{dc}[DC]{direct current}
\acrodef{ac}[AC]{alternating current}
\acrodef{ss}[SS]{spread spectrum}
\acrodef{dsss}[DSSS]{direct sequence \aclu{ss}}
\acrodef{fhss}[FHSS]{frequency hopping \aclu{ss}}
\acrodef{gps}[GPS]{global positioning system}
\acrodef{ap}[AP]{access point}
\acrodef{rts}[RTS]{request to send}
\acrodef{cts}[CTS]{clear to send}
\acrodef{macaw}[MACAW]{multiple access collision avoidance for wireless}
\acrodef{sifs}[SIFS]{short interframe space}
\acrodef{ssid}[SSID]{service set identifier}
\acrodef{mu}[MU]{multi-user}
\acrodef{mumimo}[MU-MIMO]{multi-user multiple-input-multiple-output}
\acrodef{sta}[STA]{station}
\acrodef{wcsp}[WCSP]{Wireless Communications and Signal Processing}
\acrodef{metu}[METU]{Middle East Technical University}
\acrodef{njit}[NJIT]{New Jersey Institute of Technology}
\acrodef{usf}[USF]{University of South Florida}
\acrodef{nnrp}[NNRP]{network normalized received power}
\acrodef{mrc}[MRC]{maximum ratio combining}
\acrodef{uci}[UCI]{uplink channel information}
\acrodef{map}[MAP]{maximum a posteriori}
\acrodef{ls}[LS]{least squares}
\acrodef{mai}[MAI]{multiple access interference}
\acrodef{gmm}[GMM]{Gaussian mixture model}
\acrodef{pca}[PCA]{principal component analysis}
\acrodef{prb}[PRB]{physical resource block}
\acrodef{tti}[TTI]{transmission time interval}
\acrodef{tdl}[TDL]{tapped delay line}
\acrodef{llr}[LLR]{log-likelihood ratio}
\acrodef{re}[RE]{resource element}
\acrodef{gnb}[gNB]{next generation NodeB}
\acrodef{pusch}[PUSCH]{physical uplink shared channel}
\acrodef{psd}[PSD]{power spectral density}
\acrodef{dmrs}[DMRS]{demodulation reference signal}
\acrodef{bch}[BCH]{Bose–Chaudhuri–Hocquenghem} % \cite{Bose1960} \cite{Hocquenghem1959}
\acrodef{sg}[SG]{subcarrier group}
\acrodef{bwp}[BWP]{bandwidth part}
\acrodef{tpc}[TPC]{Turbo product code}
\acrodef{pam}[PAM]{pulse amplitude modualation}
\acrodef{lmmse}[LMMSE]{linear minimum mean square error}
\acrodef{ofdmim}[OFDM-IM]{OFDM with index modulation}
\acrodef{pd_noma}[PD-NOMA]{power-domain NOMA}
\acrodef{ldpc}[LDPC]{low-density parity-check}
\acrodef{otfs}[OTFS]{orthogonal time frequency space}
\acrodef{irs}[IRS]{intelligent reflecting surface}
\acrodef{los}[LOS]{line-of-sight}
\acrodef{nlos}[NLOS]{non-line-of-sight}
\acrodef{lis}[LIS]{large intelligent surface}
\acrodef{ris}[RIS]{reconfigurable intelligent surface}
\acrodef{pim}[PIM]{passive intelligent mirrors}
\acrodef{bpl}[BPL]{building penetration loss}
\acrodef{upa}[UPA]{uniform planar array}
\acrodef{ura}[URA]{uniform rectangular array}
\acrodef{ula}[ULA]{uniform linear array}
\acrodef{aoa}[AoA]{angle-of-arrival}
\acrodef{aod}[AoD]{angle-of-departure}
\acrodef{as}[AS]{angular spread}
\acrodef{af}[AF]{array factor}
\acrodef{ple}[PLE]{pathloss exponent}
\acrodef{sf}[SF]{shadow fading}
\acrodef{ccdf}[CCDF]{complementary cumulative distribution function}
\acrodef{pmcw}[PMCW]{phase-modulated continuous wave}
\acrodef{fmcw}[FMCW]{frequency modulated continuous-wave}
\acrodef{cpi}[CPI]{coherent processing interval}
\acrodef{rcs}[RCS]{radar cross section}
\acrodef{jrc}[JRC]{joint radar-communication}
\acrodef{jcr}[JCR]{joint communication-radar}
\acrodef{dsp}[DSP]{digital signal processing}
\acrodef{lmmse}[LMMSE]{linear minimum mean square error}
\acrodef{blue}[BLUE]{best linear unbiased estimator}
\acrodef{fir}[FIR]{finite impulse response}
\acrodef{sdr}[SDR]{software-defined radio}
\acrodef{apsl}[APSL]{auto-correlation peak sidelobe level}
\acrodef{cpl}[CPL]{cross-correlation peak level}
\acrodef{musa}[MUSA]{multi-user shared access}
\acrodef{crlb}[CRLB]{Cram{\'e}r-Rao lower bound}

==> acros.tex <==
% Extend acronym package with first letter caps
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother
% Acronyms
\acrodef{ofdm}[OFDM]{orthogonal frequency division multiplexing}
\acrodef{fofdm}[F-OFDM]{filtered-\aclu{ofdm}}
\acrodef{fbmc}[FBMC]{filter bank multicarrier}
\acrodef{fmt}[FMT]{filtered multitone}
\acrodef{ufmc}[UFMC]{universal filtered multicarrier}
\acrodef{gfdm}[GFDM]{generalized frequency division multiplexing}
\acrodef{zf}[ZF]{zero forcing}
\acrodef{mimo}[MIMO]{multiple-input multiple-output}
\acrodef{siso}[SISO]{single-input single-output}
\acrodef{np}[NP]{nondeterministic polynomial}
\acrodef{sc}[SC]{single carrier}
\acrodef{sc-fde}[SC-FDE]{\aclu{sc}-\aclu{fde}}
\acrodef{evm}[EVM]{error vector magnitude}
\acrodef{dft}[DFT]{discrete Fourier transformation}
\acrodef{ifft}[IFFT]{inverse fast Fourier transformation}
\acrodef{cp}[CP]{cyclic prefix}
\acrodef{papr}[PAPR]{peak-to-average power ratio}
\acrodef{qam}[QAM]{quadrature amplitude modulation}
\acrodef{ask}[ASK]{amplitude shift keying}
\acrodef{psk}[PSK]{phase shift keying}
\acrodef{apsk}[APSK]{amplitude phase shift keying}
\acrodef{fsk}[FSK]{frequency shift keying}
\acrodef{gmsk}[GMSK]{gaussian minimum shift keying}
\acrodef{im}[IM]{index modulation}
\acrodef{fft}[FFT]{fast Fourier transformation}
\acrodef{ici}[ICI]{inter-carrier interference}
\acrodef{isi}[ISI]{intersymbol interference}
\acrodef{ini}[INI]{inter-numerology interference}
\acrodef{pdf}[PDF]{probability density function}
\acrodef{cr}[CR]{cognitive radio}
\acrodef{wola}[WOLA]{weighted overlap-add}
\acrodef{qos}[QoS]{Quality of Service}
\acrodef{csi}[CSI]{channel state information}
\acrodef{ber}[BER]{bit-error rate}
\acrodef{rf}[RF]{radio frequency}
\acrodef{rrc}[RRC]{root-raised cosine}
\acrodef{as}[AS]{alignment signal}
\acrodef{snr}[SNR]{signal-to-noise ratio}
\acrodef{dfe}[DFE]{decision-feedback equalizer}
\acrodef{fde}[FDE]{frequency domain equalization}
\acrodef{oob}[OOB]{out-of-band}
\acrodef{aci}[ACI]{adjacent channel interference}
\acrodef{naci}[NACI]{noise-plus-\aclu{aci}}
\acrodef{phy}[PHY]{physical layer}
\acrodef{mse}[MSE]{mean-square error}
\acrodef{pa}[PA]{power amplifier}
\acrodef{rb}[RB]{resource block}
\acrodef{ran}[RAN]{radio-access network}
\acrodef{rat}[RAT]{radio access technology}
\acrodefplural{rat}[RATs]{radio access technologies}
\acrodef{mmwave}[mmWave]{millimeter wave}
\acrodef{3gpp}[3GPP]{Third Generation Partnership Project}
\acrodef{sc}[SC]{single carrier}
\acrodef{uw}[UW]{unique word}
\acrodef{zt}[ZT]{zero tail}
\acrodef{gi}[GI]{guard interval}
\acrodef{sinr}[SINR]{signal to interference plus noise ratio}
\acrodef{dpss}[DPSS]{discrete prolate spheroidal sequences}
\acrodef{bler}[BLER]{block error rate}
\acrodef{fdd}[FDD]{frequency domain duplexing}
\acrodef{tdd}[TDD]{time domain duplexing}
\acrodef{ul}[UL]{uplink}
\acrodef{dl}[DL]{downlink}
\acrodef{bs}[BS]{base station}
\acrodef{af}[AF]{ambiguity function}
\acrodef{ms}[MS]{mobile station}
\acrodef{iot}[IoT]{Internet of Things}
\acrodef{pdp}[PDP]{power delay profile}
\acrodef{ftn}[FTN]{Faster-than-Nyquist}
\acrodef{svd}[SVD]{singular-value decomposition}
\acrodef{uw-ofdm}[UW-OFDM]{\aclu{uw}-\aclu{ofdm}}
\acrodef{w-ofdm}[W-OFDM]{windowed-\aclu{ofdm}}
\acrodef{rw-ofdm}[RW-OFDM]{receiver \aclu{w-ofdm}}
\acrodef{cp-ofdm}[CP-OFDM]{\aclu{cp}-\aclu{ofdm}}
\acrodef{dft-s-ofdm}[DFT-s-OFDM]{\aclu{dft}-spread-\aclu{ofdm}}
\acrodef{lte}[LTE]{Long Term Evolution}
\acrodef{lte-a}[LTE-A]{\aclu{lte}-Advanced}
\acrodef{gsm}[GSM]{Global System for Mobile Communications}
\acrodef{ma}[MA]{multiple accessing}
\acrodef{oma}[OMA]{orthogonal multiple access}
\acrodef{noma}[NOMA]{non-orthogonal multiple access}
\acrodef{cdnoma}[CD-NOMA]{code domain \aclu{noma}}
\acrodef{pdnoma}[PD-NOMA]{power domain \aclu{noma}}
\acrodef{fdma}[FDMA]{frequency division multiple accessing}
\acrodef{ofdma}[OFDMA]{orthogonal frequency division multiple accessing}
\acrodef{sc-fdma}[SC-FDMA]{single carrier-frequency division multiple accessing}
\acrodef{cdma}[CDMA]{code division multiple access}
\acrodef{tdma}[TDMA]{time division multiple access}
\acrodef{embb}[eMBB]{enhanced-mobile broadband}
\acrodef{mmtc}[mMTC]{massive machine type communications}
\acrodef{urllc}[uRLLC]{ultra-reliable and low-latency communications}
\acrodef{dvb}[DVB]{digital video broadcasting}
\acrodef{comp}[CoMP]{Coordinated Multi Point}
\acrodef{jt-comp}[JT-CoMP]{Joint Transmission-\aclu{comp}}
\acrodef{sic}[SIC]{successive interference cancellation}
\acrodef{osic}[OSIC]{ordered successive interference cancellation}
\acrodef{ml}[ML]{maximum likelihood}
\acrodef{mud}[MUD]{multi-user detection}
\acrodef{mlmud}[ML-MUD]{maximum likelihood multi-user detection}
\acrodef{sl}[SL]{sidelink}
\acrodef{qpsk}[QPSK]{quadrature phase shift keying}
\acrodef{mpa}[MPA]{message passing algorithm}
\acrodef{amc}[AMC]{adaptive modulation and coding}
\acrodef{umts}[UMTS]{Universal Mobile Telecommunications Service}
\acrodef{e-utra}[E-UTRA]{Evolved \aclu{umts} Terrestrial Radio Access}
\acrodef{ue}[UE]{user equipment}
\acrodef{harq}[HARQ]{hybrid automatic repeat request}
\acrodef{nr}[NR]{new radio}
\acrodef{hetnet}[HetNet]{heterogeneous network}
\acrodef{pot}[POT]{partially overlapping tones}
\acrodef{rms}[RMS]{root mean square}
\acrodef{must}[MUST]{multiuser superposition transmission}
\acrodef{csma}[CSMA]{carrier sense \aclu{ma}}
\acrodef{sdma}[SDMA]{space division \aclu{ma}}
\acrodef{mno}[MNO]{mobile network operator}
\acrodef{d2d}[D2D]{device-to-device}
\acrodef{v2v}[V2V]{vehicle-to-vehicle}
\acrodef{v2x}[V2X]{vehicle-to-infrastructure}
\acrodef{med}[MED]{maximum excess delay}
\acrodef{awgn}[AWGN]{additive white Gaussian noise}
\acrodef{cfr}[CFR]{channel frequency response}
\acrodef{cir}[CIR]{channel impulse response}
\acrodef{sir}[SIR]{signal-to-interference ratio}
\acrodef{lut}[LUT]{lookup table}
\acrodef{ssw}[SSW]{subcarrier specific window}
\acrodef{cqi}[CQI]{channel quality indicator}
\acrodef{bpsk}[BPSK]{binary phase shift keying}
\acrodef{mcs}[MCS]{modulation and coding scheme}
\acrodef{dac}[DAC]{digital-to-analog converter}
\acrodef{ncofdm}[NC-OFDM]{$N$-Continuous \aclu{ofdm}}
\acrodef{adc}[ADC]{analog-to-digital converter}
\acrodef{e2e}[E2E]{end-to-end}
\acrodef{kpi}[KPI]{key performance indicator}
\acrodef{p1db}[P1dB]{1 dB compression point}
\acrodef{sqnr}[SQNR]{signal-to-quantization-noise ratio}
\acrodef{cmos}[CMOS]{complementary metal–oxide–semiconductor}
\acrodef{cs}[CS]{cyclic suffix}
\acrodef{pn}[PN]{phase noise}
\acrodef{xo}[XO]{crystal oscillator}
\acrodef{dc}[DC]{direct current}
\acrodef{ac}[AC]{alternating current}
\acrodef{ss}[SS]{spread spectrum}
\acrodef{dsss}[DSSS]{direct sequence \aclu{ss}}
\acrodef{fhss}[FHSS]{frequency hopping \aclu{ss}}
\acrodef{gps}[GPS]{global positioning system}
\acrodef{ap}[AP]{access point}
\acrodef{rts}[RTS]{request to send}
\acrodef{cts}[CTS]{clear to send}
\acrodef{macaw}[MACAW]{multiple access collision avoidance for wireless}
\acrodef{sifs}[SIFS]{short interframe space}
\acrodef{ssid}[SSID]{service set identifier}
\acrodef{mu}[MU]{multi-user}
\acrodef{mumimo}[MU-MIMO]{multi-user multiple-input-multiple-output}
\acrodef{sta}[STA]{station}
\acrodef{wcsp}[WCSP]{Wireless Communications and Signal Processing}
\acrodef{metu}[METU]{Middle East Technical University}
\acrodef{njit}[NJIT]{New Jersey Institute of Technology}
\acrodef{usf}[USF]{University of South Florida}
\acrodef{nnrp}[NNRP]{network normalized received power}
\acrodef{mrc}[MRC]{maximum ratio combining}
\acrodef{uci}[UCI]{uplink channel information}
\acrodef{map}[MAP]{maximum a posteriori}
\acrodef{ls}[LS]{least squares}
\acrodef{mai}[MAI]{multiple access interference}
\acrodef{gmm}[GMM]{Gaussian mixture model}
\acrodef{pca}[PCA]{principal component analysis}
\acrodef{prb}[PRB]{physical resource block}
\acrodef{tti}[TTI]{transmission time interval}
\acrodef{tdl}[TDL]{tapped delay line}
\acrodef{llr}[LLR]{log-likelihood ratio}
\acrodef{re}[RE]{resource element}
\acrodef{gnb}[gNB]{next generation NodeB}
\acrodef{pusch}[PUSCH]{physical uplink shared channel}
\acrodef{psd}[PSD]{power spectral density}
\acrodef{dmrs}[DMRS]{demodulation reference signal}
\acrodef{bch}[BCH]{Bose–Chaudhuri–Hocquenghem} % \cite{Bose1960} \cite{Hocquenghem1959}
\acrodef{sg}[SG]{subcarrier group}
\acrodef{bwp}[BWP]{bandwidth part}
\acrodef{tpc}[TPC]{Turbo product code}
\acrodef{pam}[PAM]{pulse amplitude modualation}
\acrodef{lmmse}[LMMSE]{linear minimum mean square error}
\acrodef{ofdmim}[OFDM-IM]{OFDM with index modulation}
\acrodef{pd_noma}[PD-NOMA]{power-domain NOMA}
\acrodef{ldpc}[LDPC]{low-density parity-check}
\acrodef{otfs}[OTFS]{orthogonal time frequency space}
\acrodef{irs}[IRS]{intelligent reflecting surface}
\acrodef{los}[LOS]{line-of-sight}
\acrodef{nlos}[NLOS]{non-line-of-sight}
\acrodef{lis}[LIS]{large intelligent surface}
\acrodef{ris}[RIS]{reconfigurable intelligent surface}
\acrodef{pim}[PIM]{passive intelligent mirrors}
\acrodef{bpl}[BPL]{building penetration loss}
\acrodef{upa}[UPA]{uniform planar array}
\acrodef{ura}[URA]{uniform rectangular array}
\acrodef{ula}[ULA]{uniform linear array}
\acrodef{aoa}[AoA]{angle-of-arrival}
\acrodef{aod}[AoD]{angle-of-departure}
\acrodef{as}[AS]{angular spread}
\acrodef{af}[AF]{array factor}
\acrodef{ple}[PLE]{pathloss exponent}
\acrodef{sf}[SF]{shadow fading}
\acrodef{ccdf}[CCDF]{complementary cumulative distribution function}
\acrodef{pmcw}[PMCW]{phase-modulated continuous wave}
\acrodef{fmcw}[FMCW]{frequency modulated continuous-wave}
\acrodef{cpi}[CPI]{coherent processing interval}
\acrodef{rcs}[RCS]{radar cross section}
\acrodef{jrc}[JRC]{joint radar-communication}
\acrodef{jcr}[JCR]{joint communication-radar}
\acrodef{dsp}[DSP]{digital signal processing}
\acrodef{lmmse}[LMMSE]{linear minimum mean square error}
\acrodef{blue}[BLUE]{best linear unbiased estimator}
\acrodef{fir}[FIR]{finite impulse response}
\acrodef{sdr}[SDR]{software-defined radio}
\acrodef{apsl}[APSL]{auto-correlation peak sidelobe level}
\acrodef{cpl}[CPL]{cross-correlation peak level}
\acrodef{musa}[MUSA]{multi-user shared access}
\acrodef{crlb}[CRLB]{Cram{\'e}r-Rao lower bound}
